A Visual Active Search Framework for Geospatial Exploration

Many problems can be viewed as forms of geospatial search aided by aerial imagery, with examples ranging from detecting poaching activity to human trafficking. We model this class of problems in a visual active search (VAS) framework, which has three key inputs: (1) an image of the entire search area, which is subdivided into regions, (2) a local search function, which determines whether a previously unseen object class is present in a given region, and (3) a fixed search budget, which limits the number of times the local search function can be evaluated. The goal is to maximize the number of objects found within the search budget. We propose a reinforcement learning approach for VAS that learns a meta-search policy from a collection of fully annotated search tasks. This meta-search policy is then used to dynamically search for a novel target-object class, leveraging the outcome of any previous queries to determine where to query next. Through extensive experiments on several large-scale satellite imagery datasets, we show that the proposed approach significantly outperforms several strong baselines. We also propose novel domain adaptation techniques that improve the policy at decision time when there is a significant domain gap with the training data. Code is publicly available.

==> intro1.tex <==
\vspace{-14pt}
\section{Introduction}
\vspace{-2pt}

  %Consider a large national park that hosts endangered animals, which are also in high demand on a black market, creating a major poaching problem.
  %An important strategy in an anti-poaching portfolio is to obtain aerial imagery using drones that helps detect poaching activity, either ongoing, or in the form of traps laid on the ground~\cite{bondi2018airsim,bondi2018spot,bondi2020birdsai,fang2015security,fang2016deploying}.
  %The quality of the resulting photographs, however, is generally somewhat poor, making the detection problem extremely difficult.
  %Moreover, park rangers can only inspect relatively few small regions to confirm poaching activity, doing so sequentially.
  %Crucially, inspecting such regions yields \emph{new ground truth} information about poaching activity that we can use to decide which regions to inspect in the future.
  %We can distill some key generalizable structure from this scenario: given a broad area image (often with a relatively low resolution), \emph{sequentially query} small areas within it (e.g., by sending park rangers to the associated regions, on the ground), with each query returning the ground truth, to identify as many target objects (e.g., poachers or traps) as possible.
  %The number of queries we can make is typically limited, for example, by budget or resource constraints.
  %Moreover, query results (e.g., detected poaching activity in a particular region) are \emph{highly informative about the locations of target objects in other regions}, for example, due to spatial correlation.
  %We refer to this general modeling framework as \emph{visual active search (VAS)}.
  %Numerous other scenarios share this broad structure, such as identification of drug or human trafficking sites, broad area search-and-rescue, identifying landmarks, and many others.

\textcolor{blue}{The increasing availability of overhead imagery, often captured using drones or satellites, provides a valuable resource for geospatial search tasks. Various domains, including search and rescue, anti-poaching efforts, drug trafficking, and migration tracking increasingly require time sensitive verification of results.  This can be due to the poor quality of such images, the difficulty of automated object detection, or the cost and effort that arises once a detection occurs. Moreover, resources for verification are typically limited, so it's crucial to prioritize the areas that are most likely to contain the target objects. In this context, the typical object detection approach, which greedily analyzes the most likely areas first, may not be ideal. Because objects can move over time, a more dynamic and adaptive approach is needed—one that leverages the informative nature of past search results to guide future queries more effectively. We refer to this problem as \emph{visual active search (VAS)}, a modeling framework in which we sequentially query small areas within a broad area image to identify target objects. The results of each query provide new ground truth information, which can be highly informative about the locations of target objects in other regions, due to spatial correlation. In this paper, we address the challenges of VAS in the context of geospatial search with temporal constraints, and propose a new method that takes into account the dynamic nature of the objects being searched.}





 %While computer vision tasks on aerial overhead imagery have expanded greatly in recent years, focus has been on classification, semantic segmentation, and object detection. While attempts have been made to utilize these methods to find objects in large overhead imagery, they have often been found to be expensive as they require high quality labeled data to perform well. It is usually trivial to aquire large amounts of overhead imagery, but in almost all cases it is cumbersome and difficult to label this data, as it involves human labor. Labeled data then often needs reviewed and relabeled due to human error in labeling objects that may compose only a handful of pixels or be occluded by shadows and other confusers. Moreover, large geographic areas are costly to exhaustively search. For even a relatively small area, a search may require thousands of sub images to be manually viewed or otherwise analyzed. For these reasons, we seek to design an adaptive search strategy that learns a policy by sequential sub region queries under a search budget. We call this search strategy VAS.
 
 %For this reason, it is desirable to design an adaptive policy that learns to query image sub-regions sequentially in order to discover as many target sub-regions as possible within a limited budget on unlabeled data at a future time. 
 
 %To this end, we introduce a sequential Visual Active Search policy (VAS). 
 
 
\begin{figure}
 \centering
 \includegraphics[width=.8\linewidth]{fig_nbj/figure1.jpg}
 
 \caption{A comparison of a greedy search policy (dashed line) with an active search strategy (solid line) for the \emph{small car} target class. The greedy policy is not able to adapt when a car is not found in the starting cell and needlessly searches many similar cells. The active strategy adapts and explores regions with different visual characteristics, eventually finding the objects of interest.
  }
 
 \vspace{-10pt}
 \label{fig:introduction}
\end{figure}

A simple solution to the broad-area search problem is to divide the broad area into many grid cells, train a classifier to predict existence of a target object in each grid cell (or use object detection, segmentation, etc.~for this purpose), and simply explore the top $K$ cells in terms of predicted likelihood of the object being in the cell.
We call this the \emph{greedy} policy, which essentially reduces geospatial active search to the familiar \emph{object detection} problem.

%Suppose we look for small cars in an image, and consider cells 1 and 2, or 3 and 4, which contain water (and, consequently, no cars).
%If we can learn spatial correlation patterns in images, then exploring grid cell 1 and finding no car also suggests that no car is likely in cell 2; similar logic applies in cells 3 and 4.
Suppose we look for small cars in an image, starting in the grid marked \emph{start}, which we initially think is the best place to look.
%Many cells which contain grass-field (and, consequently, no cars). 

%%currently in draft
%In Figure~\ref{fig:introduction}, we offer some intuition about why this idea fails to capture important problem structure.
%The greedy policy would be to continuing exploring similar regions, because they are most likely to contain the target object. 
%What this approach ignores, as does framing the problem as object detection, is the fact that both success and failure of past queries is informative; here, because the car was not found, we proceed to instead explore regions that have somewhat different characteristics.




\textcolor{blue}{A greedy policy will view the most likely grid sequentially from most likely to least likely until its search budget is exhausted. When a query is made the result from this query does not affect (or reorder) the remaining grids to be searched. What this approach ignores, as does framing the problem as object detection, is the fact that both success and failure of past queries is informative. Images that a greedy search thinks are likely to have an object are likely to be very similar. Failure to find an object in an area that was previously believed to have a high likelihood of containing objects should prompt us to adjust our belief about other similar areas. As such this type of heuristic is well known to not necessarily lead to the optimal solution \cite[p.~423]{CLRS}. We demonstrate this behavior in figure~\ref{fig:introduction}, which offers some intuition about why a greedy policy may fail to capture information over queries. }






%What we propose is to adjust which image region to explore next depending on whether an object was found in the previously explored cell(s). In this case, because a car was not found we instead explore a region with different visual characteristics. We repeat this process and eventually discover the image regions that contain the desired object type.
%
%
% If we can learn spatial correlation patterns in images, then exploring the starting cell and finding no car also suggests that no car is likely in path marked by the dashed arrow. Similar logic applies to finding cars via the path marked with the solid arrow.
%In other words, the fact that we obtain \emph{ground truth} over a sequence of exploration steps (or queries, as we refer to these henceforth) can be extremely informative if we have learned how to use this information during training.
The key to visual active search, therefore, is to learn how to make use of the ground truth information obtained over a sequence of queries to decide where to query next.

 %Now, one naive approach to tackle the problem at hand, is to search greedily, i.e., select top $K$ (assuming a search budget $K$) most probable target regions at once. Such a greedy approach fails to utilize the extra information available from all the previous queries. We provide an illustrative visualization in figure ~\ref{fig:introduction} to show the importance of sequential Visual Active Search strategy (VAS). Assume that VAS selects $x^{(1)}$ to query and, as an outcome, receives a negative reward because that particular grid doesn't contain any target items. Note that although querying $x^{(1)}$  yields no immediate benefit, it aids in overall search performance  as it will no longer consider searching  $x^{(2)},x^{(4)},$ and $x^{(5)}$. This is because $x^{(1)},x^{(2)},x^{(4)},$ and $x^{(5)}$ are highly correlated. This example exemplifies the type of nontrivial decisions that a Bellman optimal policy can make. Even if the probability of finding an object is higher in some grid, it may be optimal to search a more low propensity grid if it means eliminating all grids correlated to it. On the other hand, let's assume at a particular juncture in the search process, $x^{(6)}$ is the one that VAS chooses to query, and as a result, it is rewarded favorably because it contains one or more target items. Such observation contemplates VAS to query similar grids to discover additional target objects (see path from $x^{(6)}$  to $x^{(7)}$ in figure~\ref{fig:introduction}). 

\noindent
\textbf{Relationship to Active Search and Active Learning}
\emph{VAS} is closely related to \emph{active search}~\cite{garnett2012bayesian,garnett2015introducing,jiang2017efficient,jiang2019cost}.
Active search is typically concerned with binary classification, and aims to maximize the number of discovered positively-labeled inputs.
It uses a function $f$, which predicts labels of inputs $x$, as a means to this end, with each query serving the dual-purpose of improving $f$ as well as identifying a positive instance.
A central concern in active search, therefore, is achieving a balance of exploration (learning $f$) and exploitation (identifying target inputs).
%: the goals are identical, but active search conventionally begins with a predictive model $f(x)$ for a given feature vector $x$, and chooses a sequence of queries that are also used to improve the predictive efficacy of $f$.
%Thus, in active search the choice of query input vectors $x$ to query must balance exploration (improving $f$) and exploitation (maximizing the chance of identifying target inputs $x$ given $f$).
This consideration is also the key distinction between active search and \emph{active learning}~\cite{settles2012active}, which is concerned \emph{solely} with improving the predictive quality of $f$.
Thus, if we had only a single query, active learning would typically choose $x$ for which prediction is highly uncertain, whereas active search would choose $x$ for which $f(x)$ is most confidently positive. We empirically show that active learning is inappropriate for solving the active search problem.
%as in the latter we are solely concerned with improving the model $f$.

%In conventional active search, however, there is generally no training phase before a given task (defined by a set of inputs $x$ one can query).
However, current active search approaches typically lack a pre-search training phase, and are therefore effective in relatively low dimensions and for relatively simple model classes such as $k$-nearest-neighbors.
%However, current active search approaches typically lack a pre-search training phase, and are therefore ineffective in relatively high dimension input spaces as we demonstrate later.
In \emph{VAS}, in contrast, our goal is to \emph{learn how to search}, that is, to learn how to best use information obtained from previous search queries in choosing the next query.
%Moreover, \emph{VAS} problems involve reasoning based on image inputs, which implies that the domain is high-dimensional and warrants modern learning techniques; additionally, the spatial structure of the task is consequential (as illustrated above).
We experimentally demonstrate the advantage of \emph{VAS} over conventional active search below.
 
% This motivates the use of a reinforcement learning technique (RL) that learns to query grids sequentially with the objective to find maximum target object regions at termination.

\noindent
\textbf{Contributions}
We propose a deep reinforcement learning approach to solve the \emph{VAS} problem.
Our key contribution is a novel policy architecture which makes use of a natural representation of search state, in addition to the task image input, which the policy uses to dynamically adapt to the task at hand at decision time, without additional training.
Additionally, we consider a variant of \emph{VAS} in which the nature of input tasks at decision time is sufficiently different to warrant test-time adaptation, and propose several adaptation approaches that take advantage of the \emph{VAS} problem structure.
We extensively evaluate our proposed approaches to \emph{VAS} on two satellite imagery datasets in comparison with several baseline, including a state-of-the-art approach for a related problem of identifying regions of an image to zoom into~\cite{uzkent2020learning}.
Our results show that our approach significantly outperforms all baselines.

In summary, we make the following contributions:
\begin{itemize}[noitemsep,topsep=0pt]
    \item We propose \emph{visual active search (VAS)}, a novel visual reasoning model that represents an important class of geospatial exploration problems, such as identifying poaching activities, illegal trafficking, etc.
    \item We propose a deep reinforcement learning approach for \emph{VAS} that learns how to search for target objects in a broad geospatial area based on aerial imagery.
    \item We propose two new variants of \emph{test-time adaptation (TTA)} variants of \emph{VAS}: (a) \emph{Online TTA} and (b) \emph{Stepwise TTA}, as well as an improvement of the \emph{FixMatch} state-of-the-art \emph{TTA} method~\cite{sohn2020fixmatch}.
    %, and show that proposed TTA techniques further improve the efficacy of active search.
    %\item We propose a Reinforcement Learning based framework for Visual Active Search (VAS) that learns to query image sub-regions in order to discover maximum number of target regions within the search budget. 
    \item We perform extensive experiments on two publicly available satellite imagery datasets, xView and DOTA, in a variety of settings, and demonstrate that proposed approaches significantly outperform all baselines.
    %in order to validate the efficacy of our proposed method over other baselines. 
\end{itemize}
 
 
 
 
 
 %and in many cases lacking. Finding rare objects is especially difficult in overhead imagery. Objects are often very small in comparison to the whole image. Additionally, overhead imagery often features confusers ~\cite{DBLP:journals/corr/abs-2104-03510}, environmental occlusions, and shadows. Imagery is often taken at different angles, at different times of the day. Moreover, large geographic areas are costly to exhaustively search. These difficulties motivate the search for a new technique to discover rare objects in overhead imagery that is cognizant of a search budget.  VAS is such a technique the addresses all these issues as we will detail in the rest of the work. %Additionally, since this task is much harder in overhead imagery, it demonstrates a technique that solves a harder class of tasks than may be generally desired. Although not done here, this technique is general and can be easily extended to ground based imagery.


